TernGrad: Ternary Gradients to Reduce Communication in Distributed Deep Learning

High network communication cost for synchronizing gradients and parameters is the well-known bottleneck of distributed training. In this work, we propose TernGrad that uses ternary gradients to accelerate distributed deep learning in data parallelism. Our approach requires only three numerical levels {-1,0,1}, which can aggressively reduce the communication time. We mathematically prove the convergence of TernGrad under the assumption of a bound on gradients. Guided by the bound, we propose layer-wise ternarizing and gradient clipping to improve its convergence. Our experiments show that applying TernGrad on AlexNet does not incur any accuracy loss and can even improve accuracy. The accuracy loss of GoogLeNet induced by TernGrad is less than 2% on average. Finally, a performance model is proposed to study the scalability of TernGrad. Experiments show significant speed gains for various deep neural networks. Our source code is available.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


==> exp-cifar10.tex <==
\subsection{Scaling to Large Batch Size}
\label{sec:cifar10}

Using cifar-10 dataset to show that \terngrad{} can work better when the batch size grows

scaling vs. batch sizes and \# gpus (improve accuracy for large batch size?)

Show the binary gradients in TensorBoard

==> exp-mnist.tex <==
\subsection{Integrating with Various Optimizers}
\label{sec:mnist}

Using MNIST to show that \terngrad{} can work with various optimizers (gd, momentum, adam)

Some results are observed in cifar-10 (gd, adam) and imagenet (momentum).

==> tables/mnist.tex <==
\begin{table}
  \caption{ Results of \terngrad{} on \lenet{}.}
  \label{tab:mnist}
  \centering
  %\resizebox{1.0\textwidth}{!}{
  	\begin{tabular}{ccccccc}
  		\toprule
  		SGD  & base LR & total batch size  & iterations & gradients & workers\textsuperscript{$\dagger$} & accuracy\\
  		\midrule
  		\multirow{3}{*}{momentum} & \multirow{3}{*}{0.01} & \multirow{3}{*}{64}   &  \multirow{3}{*}{10K} & floating & 2 or 8 & 99.20\% \\
  		 &   &    &  & \terngrad{} & 2 & 99.22\% \\
  		 &   &    &  & \terngrad{} & 8 & 99.11\% \\
  		
  		\cmidrule{1-7}
  		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  		
  		\multirow{3}{*}{vanilla} & \multirow{3}{*}{0.1} & \multirow{3}{*}{64}   & \multirow{3}{*}{10K} & floating & 2 or 8 & 99.25\% \\
  		  &  &     &  & \terngrad{} & 2 & 99.23\% \\
  		  &  &     &  & \terngrad{} & 8 & 99.03\% \\  		
  		\bottomrule 		
  		\multicolumn{7}{l}{\textsuperscript{$\dagger$} When using floating gradients, the accuracy is the same regardless of worker number }
  	\end{tabular}
  %}
\end{table} 
